Conformal Coverage Guarantees for Any Video Temporal Grounder

Event boundaries in continuous video are ambiguous: re-annotate the same query-video pair and independent annotators mark moments that overlap by less than half on a large fraction of samples. The ground truth for video temporal grounding is therefore a distribution over intervals, yet every grounder returns a single interval with no statement of reliability, so at deployment a wrong interval is indistinguishable from a right one. COVER changes the output object: a post-hoc, model-agnostic wrapper that turns any grounder, a trained localizer or a black-box video--language model, into one that emits a temporal region containing the true moment with probability at least $1-\alpha$, by calibrating the quantile of a temporal nonconformity score on held-out labels and widening the base prediction by that amount. The guarantee is finite-sample and distribution-free under exchangeability, and requires neither retraining nor white-box access. We give two score families, a two-sided boundary-widening score for grounders that emit an interval and a super-level-set score for grounders that emit a relevance signal, and develop theory specific to grounding that bounds how large the certified region becomes, when coverage survives conditioning on event length, and how it degrades when moments from one video break exchangeability. Across three benchmarks and five grounders, realized coverage tracks the target, and calibration exposes what point metrics hide.

==> COVER-Preprint/Makefile <==
#===============================================================================
# Kurban Intelligence Lab -- paper build
#
#   make          build main.pdf (pdflatex -> bibtex -> pdflatex x2)
#   make arxiv    arxiv-submission.tar.gz, ready to upload
#   make blind    main-blind.pdf   (double-blind: no authors, no logo, no acks)
#   make logo     regenerate every logo asset from the vector master
#   make figures  regenerate the example figure
#   make clean    remove build artefacts (keeps the PDFs)
#   make purge    remove everything generated
#===============================================================================
MAIN  := main
LATEX := pdflatex -interaction=nonstopmode -halt-on-error

.PHONY: all arxiv blind logo figures clean purge
all: $(MAIN).pdf

$(MAIN).pdf: $(MAIN).tex kurbanlab.sty affiliations.tex references.bib
	$(LATEX) $(MAIN)
	-bibtex $(MAIN)
	$(LATEX) $(MAIN)
	$(LATEX) $(MAIN)
	@echo "==> $(MAIN).pdf"

# arXiv wants the .bbl, not the .bib, and no build cruft.
arxiv: $(MAIN).pdf
	@rm -rf arxiv && mkdir -p arxiv/figures arxiv/logo
	@cp $(MAIN).tex kurbanlab.sty affiliations.tex references.bib .latexmkrc $(MAIN).bbl arxiv/
	@cp figures/*.pdf arxiv/figures/ 2>/dev/null || true
	@cp logo/kil-lockup.pdf arxiv/logo/ 2>/dev/null || true
	@cd arxiv && tar czf ../arxiv-submission.tar.gz .
	@rm -rf arxiv
	@echo "==> arxiv-submission.tar.gz  (upload this)"
	@echo "    contains: $(MAIN).tex, kurbanlab.sty, affiliations.tex, $(MAIN).bbl, figures/, logo/"
	@echo "    NOT included: *.aux, *.log. references.bib IS included: arXiv ignores it,"
	@echo "    but anyone opening this tarball in Overleaf gets a working BibTeX setup."

blind:
	@sed -E 's/\\usepackage\[([^]]*)\]\{kurbanlab\}/\\usepackage[\1, blind]{kurbanlab}/' \
	     $(MAIN).tex > $(MAIN)-blind.tex
	$(LATEX) $(MAIN)-blind
	-bibtex $(MAIN)-blind
	$(LATEX) $(MAIN)-blind
	$(LATEX) $(MAIN)-blind
	@echo "==> $(MAIN)-blind.pdf  (check it: your name should appear nowhere)"

logo:
	@cd logo && sh build-logo.sh

figures:
	@cd figures && python3 make-figure.py

clean:
	@rm -f *.aux *.log *.out *.bbl *.blg *.toc *.lof *.lot *.fls *.fdb_latexmk \
	       *.synctex.gz *.nav *.snm *.vrb $(MAIN)-blind.tex
	@echo "==> cleaned"

purge: clean
	@rm -f $(MAIN).pdf $(MAIN)-blind.pdf arxiv-submission.tar.gz
	@rm -rf arxiv


==> COVER-Preprint/affiliations.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% affiliations.tex -- the lab's institution registry.
%%
%% Declare every institution the lab has ever collaborated with, ONCE, here.
%% Then copy this file into every paper. Nothing below appears in a paper unless
%% an \Author actually cites its key, and numbering is assigned in order of first
%% use -- so a solo-HBKU paper shows exactly one affiliation, numbered [1], with
%% no edits to this file.
%%
%% >>> CHECK THESE STRINGS ONCE against how your institutions want to be cited,
%% >>> then never think about them again.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% --- home ---------------------------------------------------------------------


% A second HBKU line, for co-authors who are at HBKU but not in the lab.
\DeclareAffiliation{hbku}{%
  College of Science and Engineering, Hamad Bin Khalifa University, Doha, Qatar}

% --- recurring collaborators --------------------------------------------------
\DeclareAffiliation{tamu}{%
  Department of Computer and Electrical Engineering,
  Texas A\&M University, College Station, TX, USA}

\DeclareAffiliation{iub}{%
  Luddy School of Informatics, Computing, and Engineering,
  Indiana University Bloomington, Bloomington, IN, USA}

% --- add new institutions here, never renumber anything -----------------------
\DeclareAffiliation{tamuq}{Department of Electrical and Computer Engineering, Texas A\&M University at Qatar, Doha, Qatar}
% \DeclareAffiliation{mit} {Department of ..., Massachusetts Institute of Technology, Cambridge, MA, USA}


==> Makefile <==
#===============================================================================
# Kurban Intelligence Lab -- paper build
#
#   make          build main.pdf (pdflatex -> bibtex -> pdflatex x2)
#   make arxiv    arxiv-submission.tar.gz, ready to upload
#   make blind    main-blind.pdf   (double-blind: no authors, no logo, no acks)
#   make logo     regenerate every logo asset from the vector master
#   make figures  regenerate the example figure
#   make clean    remove build artefacts (keeps the PDFs)
#   make purge    remove everything generated
#===============================================================================
MAIN  := main
LATEX := pdflatex -interaction=nonstopmode -halt-on-error

.PHONY: all arxiv blind logo figures clean purge
all: $(MAIN).pdf

$(MAIN).pdf: $(MAIN).tex kurbanlab.sty affiliations.tex references.bib
	$(LATEX) $(MAIN)
	-bibtex $(MAIN)
	$(LATEX) $(MAIN)
	$(LATEX) $(MAIN)
	@echo "==> $(MAIN).pdf"

# arXiv wants the .bbl, not the .bib, and no build cruft.
arxiv: $(MAIN).pdf
	@rm -rf arxiv && mkdir -p arxiv/figures arxiv/logo
	@cp $(MAIN).tex kurbanlab.sty affiliations.tex references.bib .latexmkrc $(MAIN).bbl arxiv/
	@cp figures/*.pdf arxiv/figures/ 2>/dev/null || true
	@cp logo/kil-lockup.pdf arxiv/logo/ 2>/dev/null || true
	@cd arxiv && tar czf ../arxiv-submission.tar.gz .
	@rm -rf arxiv
	@echo "==> arxiv-submission.tar.gz  (upload this)"
	@echo "    contains: $(MAIN).tex, kurbanlab.sty, affiliations.tex, $(MAIN).bbl, figures/, logo/"
	@echo "    NOT included: *.aux, *.log. references.bib IS included: arXiv ignores it,"
	@echo "    but anyone opening this tarball in Overleaf gets a working BibTeX setup."

blind:
	@sed -E 's/\\usepackage\[([^]]*)\]\{kurbanlab\}/\\usepackage[\1, blind]{kurbanlab}/' \
	     $(MAIN).tex > $(MAIN)-blind.tex
	$(LATEX) $(MAIN)-blind
	-bibtex $(MAIN)-blind
	$(LATEX) $(MAIN)-blind
	$(LATEX) $(MAIN)-blind
	@echo "==> $(MAIN)-blind.pdf  (check it: your name should appear nowhere)"

logo:
	@cd logo && sh build-logo.sh

figures:
	@cd figures && python3 make-figure.py

clean:
	@rm -f *.aux *.log *.out *.bbl *.blg *.toc *.lof *.lot *.fls *.fdb_latexmk \
	       *.synctex.gz *.nav *.snm *.vrb $(MAIN)-blind.tex
	@echo "==> cleaned"

purge: clean
	@rm -f $(MAIN).pdf $(MAIN)-blind.pdf arxiv-submission.tar.gz
	@rm -rf arxiv

